How Does Unlabeled Data Provably Help Out-of-Distribution Detection?

Using unlabeled data to regularize the machine learning models has demonstrated promise for improving safety and reliability in detecting out-of-distribution (OOD) data. Harnessing the power of unlabeled in-the-wild data is non-trivial due to the heterogeneity of both in-distribution (ID) and OOD data. This lack of a clean set of OOD samples poses significant challenges in learning an optimal OOD classifier. Currently, there is a lack of research on formally understanding how unlabeled data helps OOD detection. This paper bridges the gap by introducing a new learning framework SAL (Separate And Learn) that offers both strong theoretical guarantees and empirical effectiveness. The framework separates candidate outliers from the unlabeled data and then trains an OOD classifier using the candidate outliers and the labeled ID data. Theoretically, we provide rigorous error bounds from the lens of separability and learnability, formally justifying the two components in our algorithm. Our theory shows that SAL can separate the candidate outliers with small error rates, which leads to a generalization guarantee for the learned OOD classifier. Empirically, SAL achieves state-of-the-art performance on common benchmarks, reinforcing our theoretical insights. Code is publicly available at https://github.com/deeplearning-wisc/sal.

==> setup_backup.tex <==
% $I_{\text{in}}$ denote the set that contains the indices of the in-distribution data (\emph{i.e.}, $I_{\text{in}}=\{1,\ldots,n\}$)
Formally, we describe the data setup and learning goal for \model.

\textbf{Labeled in-distribution data.} Let $\mathcal{X}\subset \mathbb{R}^d$ denote the input space, $\mathcal{Y}=\{1,\ldots, K\}$ denote the label space. We assume access to a labeled training set $\mathcal{S}^{\text{in}} = \{(\*x_i, y_i)\}_{i=1}^n$, drawn \emph{i.i.d.}\ from the joint data distribution $\mathbb{P}_{\mathcal{X}\mathcal{Y}}$. Let $\mathbb{P}_{\text{in}}$ denote the marginal distribution on $\mathcal{X}$, which is also referred to as the \emph{in-distribution} (ID).  Let $\*h_{\*w}: \mathcal{X} \mapsto \mathbb{R}^K$ be a function for the classification
task with parameter $\*w$, which returns the soft classification output. Our goal is to find an optimal parameter $\*w^*$ in the hypothesis space $\mathcal{W}$ by $\*w^* = \argmin_{\*w\in \mathcal{W}} R(\*h_\*w)$, where $R_{\mathcal{S}^{\text{in}}}(\*h_\*w) =\frac{1}{n}\sum_{(\*x_i, y_i) \in \mathcal{S}^{\text{in}}} \ell (\*h_\*w(\*x_i),y_i)$ and $\ell: \mathbb{R}^{K} \times \mathcal{Y}\mapsto \mathbb{R}$ is the loss function.

\textbf{Out-of-distribution detection.} The closed-world assumption rarely holds for models deployed in the open world, where data from unknown classes can naturally emerge~\citep{bendale2015towards}. Formally, our framework concerns a common real-world scenario in which the algorithm is trained on the ID data  with classes $\mathcal{Y}$, but will then be deployed in environments containing \emph{out-of-distribution} (OOD) samples from {unknown} class $y\notin \mathcal{Y}$ and therefore should not be predicted by $\*h_{\*w}$. At its core, OOD detection estimates the lower level set $\mathcal{S} := \{\*x: \mathbb{P}_{\text{in}}(\*x) \le \beta\}$.
Given any $\*x$, it classifies $\*x$ as OOD if and only if $\*x \in \mathcal{S}$.
The threshold $\beta$ is chosen by controlling the false detection rate: $\int_{\mathcal{S}} \mathbb{P}_{\text{in}}(\*x) d\*x = 0.05$. The false rate can be chosen as a typical (\emph{e.g.}, 0.05) or another value appropriate for the application.

% As in classic statistics (see~\citep{chen2017density} and the references therein), we estimate the lower level set $\mathcal{D}$ from the ID dataset $\mathcal{S}^{\text{in}}$.


\textbf{Unlabeled wild data.} Trained on the ID data, the classifier $\*h_{\*w}$ deployed into the wild can encounter out-of-distribution data.  A major challenge in OOD detection is the lack of labeled examples of OOD. In particular, the sample space for potential OOD data can be prohibitively large, making it expensive to collect labeled OOD data. In this paper,  we incorporate unlabeled in-the-wild
samples $\mathcal{S}_{\text{wild}}=\left\{\mathbf{x}_i\right\}_{i=1}^m$ into OOD detection. These samples
potentially consist of both ID and OOD data $\mathcal{S}_{\text{wild}}^{\text{in}}$ and $\mathcal{S}_{\text{wild}}^{\text{out}}$, respectively,  and can be collected almost for free upon deploying an existing classification function (say $\*h_\*w$). Following~\cite{katzsamuels2022training}, we use the Huber contamination model~\cite{huber1992robust} to model the marginal distribution
of the wild data:
% To model the realistic environment, we consider the following characterization of the wild data following:
\begin{equation}
\mathbb{P}_\text{wild} := (1-\pi) \mathbb{P}_\text{in} + \pi \mathbb{P}_\text{out}, 
\label{eq:wild_w_cor}
\end{equation}
where $\pi \in (0,1]$.  Note that the case $\pi=0$  is
straightforward since no novelties occur and we therefore
do not consider it.

\textbf{Learning goal.} Our learning framework aims to build an OOD detector $\*g_{\boldsymbol{\theta}}:  \mathcal{X} \mapsto \mathbb{R}^2$ by leveraging data from both $\mathcal{S}^{\text{in}}$ and $\mathcal{S}_{\text{wild}}$. Specifically, it detects a set of approximate OOD samples $\mathcal{S}_{T}$ from the wild data $\mathcal{S}_{\text{wild}}$ (Section~\ref{sec:detect}) and then trains a binary classifier $\*g_{\boldsymbol{\theta}}$ with the $\mathcal{S}^{\text{in}}$ as in-distribution and $\mathcal{S}_{T}$ as OOD (Section~\ref{sec:training}). In evaluating our
model, we are interested in the following measurements:
\begin{equation}
\begin{aligned}
&(1)~\downarrow \text{FPR}(\*g_{\boldsymbol{\theta}}):=\mathbb{E}_{\*x \sim \mathbb{P}_\text{out}^\text{test}}(\mathds{1}{\{\argmax \*g_{\boldsymbol{\theta}} (\*x)=\text{in}\}}), \\
 &(2)~\uparrow \text{TPR}(\*g_{\boldsymbol{\theta}}):=\mathbb{E}_{\*x \sim \mathbb{P}_\text{in}}(\mathds{1}{\{\argmax \*g_{\boldsymbol{\theta}}(\*x)=\text{in}\}}),
\end{aligned}
\end{equation}
 where $\mathbb{P}_\text{out}^\text{test}$ denotes the OOD test distribution and "$\text{in}$" denotes the class of in-distribution. In this paper, we distinguish between the OOD
training distribution $\mathbb{P}_{\text{out}} $ and $\mathbb{P}_\text{out}^\text{test}$ since it is common in OOD detection~\cite{katzsamuels2022training}. We call the case $\mathbb{P}_{\text{out}}  = \mathbb{P}_\text{out}^\text{test}$ the \emph{stationary wild setting}   and the case with $\mathbb{P}_{\text{out}} \neq  \mathbb{P}_\text{out}^\text{test}$ the \emph{non-stationary
wild setting} and will consider both later in Section~\ref{sec:exp}.

% \section{Preliminaries} 
